From Average Effects to Targeted Assignment: A Causal Machine Learning Analysis of Swiss Active Labor Market Policies

Active labor market policies are widely used by the Swiss government, enrolling over half of all unemployed individuals. This paper evaluates the effectiveness of Swiss programs in improving employment and earnings outcomes using causal machine learning and rich administrative data on unemployed individuals in 2014 and 2015, including detailed labor market histories and other covariates. The findings for Swiss citizens and immigrants with permanent residency indicate a small positive average effect of a Temporary Wage Subsidy program on employment and earnings in the third year after program start. In contrast, Basic Courses, such as job application training, exhibit negative effects on both outcomes over the same period. No significant impacts are found for Employment Programs conducted outside the regular labor market or for Training Courses such as language or computer classes. The programs are most effective for individuals with a non-EU migration background, while Temporary Wage Subsidies also benefit those with lower educational attainment. Finally, shallow policy trees provide practical guidance for improving the targeting of program assignments.

==> Plots/CS/obs_oos_b.tex <==
\begin{table}[H]
\renewcommand{\arraystretch}{1.0} % Adjust the vertical spacing between rows
\begin{adjustbox}{width=0.65\columnwidth, center}
\captionsetup{font=large}  % Set the font size to "large"
\begin{threeparttable}
    \caption{Descriptive statistics of selected variables by program for a sample of temporary work permit, observations out of common support.}
    \centering
    \begin{tabular}{@{}lccccc@{}}
    \toprule
    \textbf{Variable} & \textbf{NP} & \textbf{TEar} & \textbf{BC} & \textbf{TC} & \textbf{TE}\\
    \midrule   
    Socio-demographic characteristics &    &   &   &   & \\
    \midrule
    age & 36.86 & 36.58 & 36.99 & 36.46 & 36.05\vspace{-0.5em}\\
    & & (3.82) & (1.69) & (5.34) & (10.20)\\
    gender (0:men) & 0.62 & 0.60 & 0.53 & 0.62 & 0.57\vspace{-0.5em}\\
    & & (4.16) & (18.05) & (0.34) & (10.29)\\
    education (1:compulsory to 6:PhD) & 3.03 & 1.99 & 2.56 & 2.45 & 1.80\vspace{-0.5em}\\
     & & (65.38) & (27.62) & (33.91) & (80.62)\\
    Proficiency local language (1:basic-7:mother tongue) & 4.58 & 4.02 & 4.50 & 2.79 & 3.67\vspace{-0.5em}\\
    & & (24.39) & (3.61) & (77.83) & (40.55)\\
    European & 0.83 & 0.67 & 0.70 & 0.67 & 0.63\vspace{-0.5em}\\
    & & (35.35) & (29.19) & (37.23) & (44.88)\\
    Rest of the world & 0.17 & 0.32 & 0.30 & 0.33 & 0.37\vspace{-0.5em}\\
     & & (35.12) & (29.19) & (37.23) & (44.88)\\
    Countries with Swiss languages & 0.42 & 0.28 & 0.38 & 0.23 & 0.21\vspace{-0.5em}\\
    & & (28.47) & (8.50) & (41.80) & (45.18)\\
    European Union & 0.36 & 0.38 & 0.31 & 0.40 & 0.42\vspace{-0.5em}\\
    & & (5.47) & (10.35) & (8.12) & (12.32)\\
    Rest of Europe & 0.04 & 0.10 & 0.09 & 0.09 & 0.09\vspace{-0.5em}\\
    & & (24.28) & (22.18) & (20.21) & (20.37)\\
    Rest of the world & 0.19 & 0.24 & 0.22 & 0.29 & 0.28\vspace{-0.5em}\\
    & & (11.75) & (8.99) & (24.54) & (22.88)\\
    Sum of months in emp. five years before  & 41.94 & 37.95 & 41.11 & 37.69 & 38.18\vspace{-0.5em}\\
     & & (29.61) & (6.08) & (29.97) & (27.72)\\
    Sum of months in emp. ten years before   & 53.92 & 50.17 & 51.23 & 45.13 & 50.51\vspace{-0.5em}\\
    & & (14.36) & (10.27) & (33.97) & (12.85)\\
    
    Sum of earning five years before  & 352,462 & 162,078 & 241,036 & 229,110 & 135,916\vspace{-0.5em}\\
    & & (58.00) & (29.60) & (34.59) & (67.25)\\
    Sum of earning ten years before & 419,965 & 205,611 & 284,746 & 270,486 & 177,765\vspace{-0.5em}\\
    & & (54.76) & (30.74) & (34.41) & (62.81)\\
  
    Sum of months in Tem. earn. five years before  & 0.99 & 2.39 & 0.39 & 0.31 & 0.85\vspace{-0.5em}\\
     & & (31.49) & (22.47) & (24.33) & (4.44)\\
    Sum of months in Tem. earn. ten years before & 1.38 & 2.90 & 0.59 & 0.41 & 1.14\vspace{-0.5em}\\
     & & (26.15) & (19.58) & (25.08) & (5.56)\\
    Sum of months in AMM ten years before & 0.69 & 1.07 & 0.45 & 0.38 & 1.26\vspace{-0.5em}\\
    & & (16.11) & (12.50) & (17.39) & (21.40)\\
    Sum of months in AMM five years before & 0.91 & 1.38 & 0.70 & 0.47 & 1.73\vspace{-0.5em}\\
    & & (16.99) & (8.86) & (20.94) & (25.19)\\
    First year credit register  & 2007 & 2007 & 2008 & 2009 & 2007\vspace{-0.5em}\\
     & & (7.94) & (6.74) & (26.88) & (11.60)\\
    \midrule
    \bottomrule
    \end{tabular}
\begin{tablenotes}
\textit{Note:} The table shows the unconditional means and Standardised differences (in brackets) for selected variables by each program. NP: Non Participation, TEar: Temporary Earnings, BC: Basic courses, TC: Training Courses, TE: Temporary Employment. Local language knowledge: from 1 to 7, from basic to mother tongue. Education: 1: Compulsory school, 2: Secondary school, 3: Diploma vocational training, 4: Bachelor degree, 5: Master degree, 6: PhD. N. of obs.: 3.338. 
\end{tablenotes}
\label{table:desc_stat_cs_dropped_b}
\end{threeparttable}
\end{adjustbox}
\end{table}


==> Plots/CS/obs_oos_swiss+.tex <==
\begin{table}[H]
\renewcommand{\arraystretch}{1.0} % Adjust the vertical spacing between rows
\begin{adjustbox}{width=0.90\columnwidth, center}
\captionsetup{font=large}  % Set the font size to "large"
\begin{threeparttable}
    \caption{Descriptive statistics of selected variables by program for samples of Swiss+ (LHS) and Temporary Work Permit (RHS) for observations out of common support.}
    \centering
    \begin{tabular}{@{}lcccccccccc@{}} \toprule
     \textbf{Variable} & \multicolumn{4}{c}{\textbf{Swiss+}} & \multicolumn{6}{c}{\textbf{Temporary Work Permit}} \\
    \midrule
     & NP & TEar & BC & TC & TE & NP & TEar & BC & TC & TE\\
    \midrule   
    Socio-demographics variables &    &   &   &   &  & & & & \\
    \midrule
    age & 37.64 & 39.25 & 39.74 & 40.63 & 39.77 & 36.86 & 36.58 & 36.99 & 36.46 & 36.05\vspace{-0.5em} \\
    & & (17.95) & (23.43) & (33.61) & (23.71) & & (3.82) & (1.69) & (5.34) & (10.20)\\
    gender (0:men) & 0.45 & 0.43 & 0.48 & 0.41 & 0.45 & 0.62 & 0.60 & 0.53 & 0.62 & 0.57\vspace{-0.5em}\\
    & & (3.17) & (6.66) & (6.95) & (0.43) & & (4.16) & (18.05) & (0.34) & (10.29)\\
    education (1:compulsory & 2.67 & 2.17 & 2.14 & 2.21 & 1.99 & 3.03 & 1.99 & 2.56 & 2.45 & 1.80\vspace{-0.5em}\\
    to 6:PhD) & & (38.56) & (41.76) & (35.43) & (56.26) & & (65.38) & (27.62) & (33.91) & (80.62) \\
    Proficiency local language  & 6.27 & 5.81 & 6.00 & 5.60 & 5.87 & 4.58 & 4.02 & 4.50 & 2.79 & 3.6\vspace{-0.5em}\\
   (1:basic-7:mother tongue) & & (26.91) & (16.72) & (36.62) & (24.04) & & (24.39) & (3.61) & (77.83) & (40.55)\\
    Swiss  & 0.76 & 0.66 & 0.64 & 0.63 & 0.66\vspace{-0.5em}\\
     & & (23.02) & (26.34) & (29.05) & (23.80)\\
    European & 0.18 & 0.19 & 0.18 & 0.21 & 0.18 & 0.83 & 0.67 & 0.70 & 0.67 & 0.63\vspace{-0.5em}\\
    & & (3.47) & (1.18) & (7.89) & (0.63)  & & (35.35) & (29.19) & (37.23) & (44.88)\\
    Rest of the world & 0.06 & 0.15 & 0.18 & 0.16 & 0.17 & 0.17 & 0.32 & 0.30 & 0.33 & 0.37\vspace{-0.5em}\\
    & & (29.67) & (36.16) & (32.59) & (33.59) & & (35.12) & (29.19) & (37.23) & (44.88)\\
    Settlement Permit & 0.24 & 0.34 & 0.36 & 0.37 & 0.34 &&&&\vspace{-0.5em}\\
    & & (22.92) & (26.55) & (28.86) & (24.01) &&&&\\
    Countries with Swiss languages & 0.84 & 0.75 & 0.75 & 0.73 & 0.74 & 0.42 & 0.28 & 0.38 & 0.23 & 0.21\vspace{-0.5em}\\
    & & (22.81) & (22.89) & (28.33) & (25.07) & & (28.47) & (8.50) & (41.80) & (45.18)\\
    European Union & 0.09 & 0.09 & 0.07 & 0.10 & 0.09 & 0.36 & 0.38 & 0.31 & 0.40 & 0.42\vspace{-0.5em}\\
    & & (1.48) & (6.94) & (2.41) & (0.27) & & (5.47) & (10.35) & (8.12) & (12.32)\\
    Rest of Europe & 0.03 & 0.07 & 0.08 & 0.05 & 0.07 & 0.04 & 0.10 & 0.09 & 0.09 & 0.09\vspace{-0.5em}\\
     & & (20.64) & (23.60) & (14.50) & (22.68) & & (24.28) & (22.18) & (20.21) & (20.37)\\
    Rest of the world & 0.04 & 0.08 & 0.10 & 0.12 & 0.09 & 0.19 & 0.24 & 0.22 & 0.29 & 0.28\\vspace{-0.5em}\\
     & & (17.79) & (22.89) & (29.52) & (20.92 & & (11.75) & (8.99) & (24.54) & (22.88))\\
     
    Sum of months in emp.  & 48.76 & 50.11 & 53.54 & 52.89 & 52.25  & 41.94 & 37.95 & 41.11 & 37.69 & 38.18\vspace{-0.5em}\\
     five years before & & (11.09) & (42.52) & (35.72) & (30.10) & & (29.61) & (6.08) & (29.97) & (27.72)\\
    Sum of months in emp. ten years before  & 91.97 & 96.95 & 94.35 & 95.26 & 53.92 & 50.17 & 51.23 & 45.13 & 50.51\vspace{-0.5em}\\
    & & (5.64) & (25.99) & (14.86) & (18.97) & & (14.36) & (10.27) & (33.97) & (12.85)\\
    Sum of earning & 302,770 & 200,557 & 269,224 & 258,325 & 215,243 & 352,462 & 162,078 & 241,036 & 229,110 & 135,916\vspace{-0.5em}\\
    five years before   & & (34.09) & (10.37) & (13.71) & (29.23) & & (58.00) & (29.60) & (34.59) & (67.25)\\
    Sum of earning  & 531,878 & 351,652 & 471,831 & 438,077 & 377,671 & 419,965 & 205,611 & 284,746 & 270,486 & 177,765\vspace{-0.5em}\\
    ten years before & & (32.72) & (10.07) & (16.15) & (28.05) & & (54.76) & (30.74) & (34.41) & (62.81)\\
    Sum of months in Tem. earn.  & 1.30 & 2.91 & 0.82 & 0.94 & 1.23 & 0.99 & 2.39 & 0.39 & 0.31 & 0.85\vspace{-0.5em}\\
    five years before & & (30.82) & (13.27) & (9.60) & (1.84) & & (31.49) & (22.47) & (24.33) & (4.44)\\
    Sum of months in Tem. earn. ten years before  & 2.08 & 4.70 & 1.77 & 2.04 & 2.45 & 1.38 & 2.90 & 0.59 & 0.41 & 1.14\vspace{-0.5em}\\
     & & (34.67) & (5.86) & (0.71) & (6.29) & & (26.15) & (19.58) & (25.08) & (5.56)\\
    Sum of months in AMM  & 1.13 & 1.07 & 0.78 & 1.12 & 1.23 & 0.69 & 1.07 & 0.45 & 0.38 & 1.26\vspace{-0.5em}\\
    ten years before & & (2.05) & (13.45) & (0.51) & (3.35) & & (16.11) & (12.50) & (17.39) & (21.40)\\
    Sum of months in AMM  & 1.69 & 1.76 & 1.53 & 1.89 & 2.10 & 0.91 & 1.38 & 0.70 & 0.47 & 1.73\vspace{-0.5em}\\
    five years before  & & (1.94) & (4.66) & (5.11) & (11.14) & & (16.99) & (8.86) & (20.94) & (25.19)\\
    First year registered & 1996 & 1996 & 1995 & 1995 & 1995 & 2007 & 2007 & 2008 & 2009 & 2007 \vspace{-0.5em}\\
    & & (8.27) & (14.92) & (14.39) & (16.00) & & (7.94) & (6.74) & (26.88) & (11.60)\\
    \bottomrule
    \end{tabular}
\begin{tablenotes}
\textit{Note:} The table shows the unconditional means and standardised differences (in brackets) for selected variables by each program. NP: Non Participation, TEar: Temporary Earnings, BC: Basic courses, TC: Training Courses, TE: Temporary Employment. Local language knowledge: from 1 to 7, from basic to mother tongue. Education: 1: Compulsory school, 2: Secondary school, 3: Diploma vocational training, 4: Bachelor degree, 5: Master degree, 6: PhD. Swiss+ sample n. of obs.: 9.549. Temporary Work Permit n. of obs.: 3.338.
\end{tablenotes}
\label{table:desc_stat_cs_dropped}
\end{threeparttable}
\end{adjustbox}
\end{table}







==> Plots/GATEs/gates_conti.tex <==
% GATEs main
\begin{figure}[H]
\captionsetup{font=small}  % Set the font size to "large"
\caption{Differences of GATEs to ATE of Temporary Earnings programs with respect to non participants to programs, Swiss+ sample.}
	\begin{minipage}[t]{0.55\textwidth}
 \includegraphics[width=0.90\textwidth]{Plots/GATEs/gate_emp1.pdf}
        %\label{fig:balance_employment}
	\end{minipage}
	\begin{minipage}[t]{0.55\textwidth}
 \includegraphics[width=0.90\textwidth]{Plots/GATEs/gate_earnings1.pdf}
	\end{minipage}
\caption*{\textit{Note:} The vertical axes measures the difference of GATEs to the ATE of Temporary Earnings Program with respect to non participants and the 95\% confidence interval. On the LHS horizontal axes the cumulative months into employment in the five years before the unemployment spell. On the RHS the cumulative earnings in the year before the start of the spell.}
\label{fig:gates_cont}
\end{figure}






==> Plots/IATEs/iates_densities.tex <==
% IATES main
\begin{figure}[H]
	\begin{minipage}[t]{0.55\textwidth}
 \includegraphics[width=0.95\textwidth]{Plots/IATEs/DensityEARN__OUTSUM2435LC1vs0_iate.pdf}
        %label{fig:iates_dens}
	\end{minipage}
	\begin{minipage}[t]{0.55\textwidth}
 \includegraphics[width=0.95\textwidth]{Plots/IATEs/DensityEARN__OUTSUM2435LC2vs0_iate.pdf}
	\end{minipage}
        \begin{minipage}[t]{0.55\textwidth}
 \includegraphics[width=0.95\textwidth]{Plots/IATEs/DensityEARN__OUTSUM2435LC3vs0_iate.pdf}
        %\label{fig:balance_employment}
	\end{minipage}
	\begin{minipage}[t]{0.55\textwidth}
 \includegraphics[width=0.95\textwidth]{Plots/IATEs/DensityEARN__OUTSUM2435LC4vs0_iate.pdf}
	\end{minipage}
\caption{\textit{Note:} The horizontal axis measures the individual average gain of participating in a program relative to NP in the cumulative earnigns in the third yea after the programs start. Up on the LHS Temporary Earnings (1) vs NP, on the RHS Basic Course (2) vs NP, LHS on the lower part Technical course (3) vs NP and Temporary Employment (4) vs NP on the RHS.  Kernel smooth with Epanechnikov Kernel and Silverman (normality) bandwidth.}
\label{fig:iates_main_dens}
\end{figure}

==> Tables/Descrip_stats/outcomes_swiss+.tex <==

\begin{table}[htbp!]\centering
    \caption{Descriptive statistics by programme: Outcome variables}
    \label{table: out_swiss+1}
    \begin{adjustbox}{max width=0.9\textwidth}
    \begin{threeparttable}

    \begin{tabular}{lrrrrrrrrrr} \toprule
    \textbf{Variable} & \multicolumn{1}{c}{NP} & \multicolumn{2}{c}{TE} & \multicolumn{2}{c}{BC} & \multicolumn{2}{c}{TC} & \multicolumn{2}{c}{TEMP} \\
        & Mean & Mean & Std. diff. & Mean & Std. diff. & Mean & Std. diff. & Mean & Std. diff. \\ \midrule
\textbf{Swiss+ sample} & & & & & & & & & \\ \midrule
Earnings first year  & 32,703 & 21,198 & (41.40)& 18,302 & (49.59)& 16,978 & (54.30) & 15,305.22 & (63.75) \\
Earnings third year & 52,053 & 44,507& (19.31) & 47,311 & (11.02)& 46,597 & (12.76)& 38742.66 & (33.84)\\
Earnings three years & 132,358 & 103,501& (31.08) & 105.585 & (26.41) & 101,997 & (30.14) & 86,891 & (48.86)\\
Months employed first year  & 5.82 & 4.50  & (32.70)  & 3.21  & (65.79) & 2.96 & (72.80) & 3.19 & (66.86)\\
Months employed third year  & 9.09 & 9.45 & (8.57) & 8.81 & (6.07) & 8.71 & (8.38) & 8.56 & (11.74)\\
Months employed three years  & 23.13  & 21.80  & (12.89)  & 19.23 & (36.60) & 18.68  & (41.71) & 18.86 & (40.36)\\ \midrule
Number of observations & 33,537 & \multicolumn{2}{c}{17,117} &\multicolumn{2}{c}{ 12,312}  &\multicolumn{2}{c}{3,745}   & \multicolumn{2}{c}{3,070}  \\\midrule 
\textbf{TW Permit sample} & & & & & & & & & \\ \midrule
Earnings first year & 27,661 & 19,155 & (34.38)& 14,989& (49.09) & 14,893 & (50.28)  & 14,264 & (54.75) \\
Earnings third year & 40,233 & 36,908& (9.67)  & 37,829& (6.31) & 39,107 & (2.95)  & 34,059 & (17.72)\\
Earnings three years & 105,438 & 87,670 & (21.78) & 85,443 & (22.48)  & 86,913 & (20.85) & 78,270 & (32.92) \\
Months employed first year & 5.37 & 4.38 & (24.86)& 2.96  & (61.91) & 2.94 & (62.92) & 3.23 & (55.07) \\
Months employed third year & 7.50 & 8.52& (21.95) & 7.93 & (8.73) & 7.95 & (9.22) & 7.94 & (9.25) \\
Months employed three years & 19.83 & 20.08 & (2.31) & 17.58  & (20.18) & 17.57  & (20.38) & 18.17 & (15.12) \\ \midrule
Number of observations & 9,076 & \multicolumn{2}{c}{5,330}  &\multicolumn{2}{c}{2,923}  &\multicolumn{2}{c}{2,021}   &\multicolumn{2}{c}{1,137}\\ \bottomrule 
\end{tabular}
    \begin{tablenotes}
        \small \item \textit{Note:} This table shows the mean and the standardised difference in comparison to the non-participants for some outcome variables by programmes for the Swiss+ and the TW Permit sample. TEarn: Temporary Earnings, BC: Basic Course, TC: Technical Course, TE: Temporary Employment, NP: No programme.
    \end{tablenotes}
    \end{threeparttable}
    \end{adjustbox}
\end{table}

==> Tables_results/GATES_tables/gates_local_lang.tex <==
%\begin{sidewaystable}
\begin{table}[H]
\renewcommand{\arraystretch}{1.2}
\begin{adjustbox}{width=0.95\columnwidth, center}
\begin{threeparttable}
  \captionsetup{font=large}
    \caption{GATE and GATEs-ATE for Proficiency in the local language}
    \centering
    \begin{tabular}{@{}lrrrrrrrrrrr| rrrrrrrrrr@{}}
    \toprule
    \textbf{Outcome-} & \textbf{Cum. Earnings} & \multicolumn{10}{c}{\textbf{First year}} & \multicolumn{10}{c}{\textbf{Third year}} \\
    \toprule
    \textbf{Programme }& \textbf{Z-value} & GATE & S.E. & S.E. & p-value & p-value & GATE-ATE & S.E.& S.E. & p-value& p-value & GATE & S.E. & S.E. & p-value& p-value& GATE-ATE & S.E.& S.E. & p-value& p-value\\
    \midrule
    1 vs. 0 & 0.0 & -5630.888 & 593.0 & 227.0 & 0.0\%**** & 17.0\% & 311.666 & 593.0 & 227.0 & 0.0\%**** & 17.0\% & 2366.937 & 947.0 & 321.0 & 1.2\%** & 9.7\%* & 532.112 & 947.0 & 321.0 & 1.2\%** & 9.7\%*\\
    1 vs. 0 & 1.0 & -4054.578 & 361.0 & 192.0 & 0.0\%**** & 0.0\%**** & 1887.975 & 361.0 & 192.0 & 0.0\%**** & 0.0\%**** & 3008.081 & 667.0 & 253.0 & 0.0\%*** & 0.0\%*** & 1173.256 & 667.0 & 253.0 & 0.0\%*** & 0.0\%***\\
    1 vs. 0 & 2.0 & -4171.071 & 397.0 & 165.0 & 0.0\%**** & 0.0\%**** & 1771.483 & 397.0 & 165.0 & 0.0\%**** & 0.0\%**** & 2963.596 & 825.0 & 222.0 & 0.0\%*** & 0.0\%*** & 1128.771 & 825.0 & 222.0 & 0.0\%*** & 0.0\%***\\
    1 vs. 0 & 3.0 & -4176.885 & 365.0 & 184.0 & 0.0\%**** & 0.0\%**** & 1765.668 & 365.0 & 184.0 & 0.0\%**** & 0.0\%**** & 3006.423 & 675.0 & 232.0 & 0.0\%*** & 0.0\%*** & 1171.598 & 675.0 & 232.0 & 0.0\%*** & 0.0\%***\\
    1 vs. 0 & 4.0 & -4447.464 & 407.0 & 142.0 & 0.0\%**** & 0.0\%**** & 1495.09 & 407.0 & 142.0 & 0.0\%**** & 0.0\%**** & 2873.709 & 866.0 & 202.0 & 0.1\%*** & 0.0\%*** & 1038.884 & 866.0 & 202.0 & 0.1\%*** & 0.0\%***\\
    1 vs. 0 & 5.0 & -4685.318 & 392.0 & 120.0 & 0.0\%**** & 0.0\%**** & 1257.235 & 392.0 & 120.0 & 0.0\%**** & 0.0\%**** & 2814.37 & 848.0 & 168.0 & 0.1\%*** & 0.0\%*** & 979.545 & 848.0 & 168.0 & 0.1\%*** & 0.0\%***\\
    1 vs. 0 & 6.0 & -5441.311 & 472.0 & 62.0 & 0.0\%**** & 0.0\%*** & 501.242 & 472.0 & 62.0 & 0.0\%**** & 0.0\%*** & 2209.288 & 848.0 & 128.0 & 0.9\%*** & 0.3\%*** & 374.463 & 848.0 & 128.0 & 0.9\%*** & 0.3\%***\\
    1 vs. 0 & 7.0 & -6469.202 & 454.0 & 47.0 & 0.0\%**** & 0.0\%**** & -526.648 & 454.0 & 47.0 & 0.0\%**** & 0.0\%**** & 1468.421 & 747.0 & 66.0 & 4.9\%** & 0.0\%*** & -366.404 & 747.0 & 66.0 & 4.9\%** & 0.0\%***\\
    2 vs. 0 & 0.0 & -10205.305 & 583.0 & 214.0 & 0.0\%**** & 31.4\% & 215.571 & 583.0 & 214.0 & 0.0\%**** & 31.4\% & -1672.899 & 976.0 & 323.0 & 8.7\%* & 57.0\% & 183.478 & 976.0 & 323.0 & 8.7\%* & 57.0\%\\
    2 vs. 0 & 1.0 & -8798.254 & 407.0 & 198.0 & 0.0\%**** & 0.0\%*** & 1622.622 & 407.0 & 198.0 & 0.0\%**** & 0.0\%*** & -479.413 & 723.0 & 274.0 & 50.7\% & 0.0\%*** & 1376.963 & 723.0 & 274.0 & 50.7\% & 0.0\%***\\
    2 vs. 0 & 2.0 & -8875.778 & 434.0 & 172.0 & 0.0\%**** & 0.0\%**** & 1545.098 & 434.0 & 172.0 & 0.0\%**** & 0.0\%**** & -577.642 & 867.0 & 241.0 & 50.5\% & 0.0\%*** & 1278.734 & 867.0 & 241.0 & 50.5\% & 0.0\%***\\
    2 vs. 0 & 3.0 & -8995.081 & 408.0 & 183.0 & 0.0\%**** & 0.0\%*** & 1425.795 & 408.0 & 183.0 & 0.0\%**** & 0.0\%*** & -568.65 & 729.0 & 249.0 & 43.6\% & 0.0\%*** & 1287.727 & 729.0 & 249.0 & 43.6\% & 0.0\%***\\
    2 vs. 0 & 4.0 & -9141.207 & 438.0 & 141.0 & 0.0\%**** & 0.0\%**** & 1279.669 & 438.0 & 141.0 & 0.0\%**** & 0.0\%**** & -735.574 & 904.0 & 211.0 & 41.6\% & 0.0\%*** & 1120.803 & 904.0 & 211.0 & 41.6\% & 0.0\%***\\
    2 vs. 0 & 5.0 & -9334.26 & 427.0 & 118.0 & 0.0\%**** & 0.0\%**** & 1086.616 & 427.0 & 118.0 & 0.0\%**** & 0.0\%**** & -832.423 & 888.0 & 177.0 & 34.8\% & 0.0\%*** & 1023.954 & 888.0 & 177.0 & 34.8\% & 0.0\%***\\
    2 vs. 0 & 6.0 & -9998.198 & 490.0 & 62.0 & 0.0\%**** & 0.0\%*** & 422.678 & 490.0 & 62.0 & 0.0\%**** & 0.0\%*** & -1543.826 & 884.0 & 130.0 & 8.1\%* & 1.6\%** & 312.551 & 884.0 & 130.0 & 8.1\%* & 1.6\%**\\
    2 vs. 0 & 7.0 & -10865.359 & 475.0 & 48.0 & 0.0\%**** & 0.0\%**** & -444.483 & 475.0 & 48.0 & 0.0\%**** & 0.0\%**** & -2240.528 & 789.0 & 70.0 & 0.5\%*** & 0.0\%*** & -384.151 & 789.0 & 70.0 & 0.5\%*** & 0.0\%***\\
    3 vs. 0 & 0.0 & -9508.639 & 778.0 & 265.0 & 0.0\%**** & 66.1\% & -116.171 & 778.0 & 265.0 & 0.0\%**** & 66.1\% & -836.318 & 1178.0 & 384.0 & 47.8\% & 64.2\% & -178.384 & 1178.0 & 384.0 & 47.8\% & 64.2\%\\
    3 vs. 0 & 1.0 & -7954.27 & 627.0 & 327.0 & 0.0\%**** & 0.0\%*** & 1438.198 & 627.0 & 327.0 & 0.0\%**** & 0.0\%*** & -148.982 & 944.0 & 427.0 & 87.5\% & 23.3\% & 508.952 & 944.0 & 427.0 & 87.5\% & 23.3\%\\
    3 vs. 0 & 2.0 & -8065.098 & 634.0 & 279.0 & 0.0\%**** & 0.0\%*** & 1327.37 & 634.0 & 279.0 & 0.0\%**** & 0.0\%*** & -141.918 & 1056.0 & 362.0 & 89.3\% & 15.4\% & 516.016 & 1056.0 & 362.0 & 89.3\% & 15.4\%\\
    3 vs. 0 & 3.0 & -8092.336 & 623.0 & 288.0 & 0.0\%**** & 0.0\%*** & 1300.131 & 623.0 & 288.0 & 0.0\%**** & 0.0\%*** & -32.65 & 938.0 & 385.0 & 97.2\% & 10.4\% & 625.283 & 938.0 & 385.0 & 97.2\% & 10.4\%\\
    3 vs. 0 & 4.0 & -8287.079 & 633.0 & 219.0 & 0.0\%**** & 0.0\%*** & 1105.389 & 633.0 & 219.0 & 0.0\%**** & 0.0\%*** & -95.66 & 1074.0 & 298.0 & 92.9\% & 5.9\%* & 562.274 & 1074.0 & 298.0 & 92.9\% & 5.9\%*\\
    3 vs. 0 & 5.0 & -8501.123 & 633.0 & 185.0 & 0.0\%**** & 0.0\%*** & 891.344 & 633.0 & 185.0 & 0.0\%**** & 0.0\%*** & 18.777 & 1060.0 & 257.0 & 98.6\% & 0.8\%*** & 676.71 & 1060.0 & 257.0 & 98.6\% & 0.8\%***\\
    3 vs. 0 & 6.0 & -9104.685 & 700.0 & 86.0 & 0.0\%**** & 0.1\%*** & 287.783 & 700.0 & 86.0 & 0.0\%**** & 0.1\%*** & -469.226 & 1083.0 & 150.0 & 66.5\% & 20.8\% & 188.707 & 1083.0 & 150.0 & 66.5\% & 20.8\%\\
    3 vs. 0 & 7.0 & -9766.631 & 730.0 & 76.0 & 0.0\%**** & 0.0\%*** & -374.163 & 730.0 & 76.0 & 0.0\%**** & 0.0\%*** & -846.843 & 1037.0 & 101.0 & 41.4\% & 6.1\%* & -188.909 & 1037.0 & 101.0 & 41.4\% & 6.1\%*\\
    4 vs. 0 & 0.0 & -9051.341 & 981.0 & 306.0 & 0.0\%**** & 10.9\% & 490.178 & 981.0 & 306.0 & 0.0\%**** & 10.9\% & -1109.5 & 1317.0 & 416.0 & 39.9\% & 11.4\% & 658.419 & 1317.0 & 416.0 & 39.9\% & 11.4\%\\
    4 vs. 0 & 1.0 & -6863.544 & 657.0 & 417.0 & 0.0\%**** & 0.0\%*** & 2677.975 & 657.0 & 417.0 & 0.0\%**** & 0.0\%*** & 449.447 & 958.0 & 497.0 & 63.9\% & 0.0\%*** & 2217.367 & 958.0 & 497.0 & 63.9\% & 0.0\%***\\
    4 vs. 0 & 2.0 & -7104.271 & 670.0 & 364.0 & 0.0\%**** & 0.0\%*** & 2437.248 & 670.0 & 364.0 & 0.0\%**** & 0.0\%*** & 243.185 & 1070.0 & 426.0 & 82.0\% & 0.0\%*** & 2011.105 & 1070.0 & 426.0 & 82.0\% & 0.0\%***\\
    4 vs. 0 & 3.0 & -7180.426 & 656.0 & 382.0 & 0.0\%**** & 0.0\%*** & 2361.093 & 656.0 & 382.0 & 0.0\%**** & 0.0\%*** & 185.786 & 963.0 & 452.0 & 84.7\% & 0.0\%*** & 1953.706 & 963.0 & 452.0 & 84.7\% & 0.0\%***\\
    4 vs. 0 & 4.0 & -7688.061 & 688.0 & 296.0 & 0.0\%**** & 0.0\%*** & 1853.457 & 688.0 & 296.0 & 0.0\%**** & 0.0\%*** & -115.153 & 1107.0 & 352.0 & 91.7\% & 0.0\%*** & 1652.767 & 1107.0 & 352.0 & 91.7\% & 0.0\%***\\
    4 vs. 0 & 5.0 & -7896.364 & 708.0 & 249.0 & 0.0\%**** & 0.0\%*** & 1645.155 & 708.0 & 249.0 & 0.0\%**** & 0.0\%*** & -187.478 & 1107.0 & 298.0 & 86.6\% & 0.0\%*** & 1580.442 & 1107.0 & 298.0 & 86.6\% & 0.0\%***\\
    4 vs. 0 & 6.0 & -9011.382 & 830.0 & 101.0 & 0.0\%**** & 0.0\%*** & 530.137 & 830.0 & 101.0 & 0.0\%**** & 0.0\%*** & -1123.339 & 1173.0 & 157.0 & 33.8\% & 0.0\%*** & 644.581 & 1173.0 & 157.0 & 33.8\% & 0.0\%***\\
    4 vs. 0 & 7.0 & -10219.034 & 901.0 & 102.0 & 0.0\%**** & 0.0\%*** & -677.515 & 901.0 & 102.0 & 0.0\%**** & 0.0\%*** & -2378.217 & 1163.0 & 120.0 & 4.1\%** & 0.0\%*** & -610.298 & 1163.0 & 120.0 & 4.1\%** & 0.0\%***\\
    \bottomrule
    \end{tabular}
\end{threeparttable}
\end{adjustbox}
\end{table}
%\end{sidewaystable}

==> Tables_results/GATES_tables/gates_permit_type.tex <==
\begin{table}[htbp!]
\begin{adjustbox}{width=0.95\columnwidth, center}
\begin{threeparttable}
  \captionsetup{font=large}
    \caption{GATEs for Permit type, Swiss+ sample}
    \label{table:gate_permit_type}
    \centering
    \begin{tabular}{@{}ll|rrrrrr|rrrrrrr@{}}
    \toprule
    \multicolumn{2}{l}{\textbf{Permit type}}& \multicolumn{6}{c}{\textbf{First Year}} & \multicolumn{6}{c}{\textbf{Third Year}} \\
    \midrule
     & Programme & GATE & S.E. & p-value & GATE-ATE & S.E. & p-value & GATE & S.E. & p-value & GATE-ATE & S.E. & p-value \\
    \midrule
    &&  \multicolumn{12}{c}{\textbf{Outcome: Employment}} \\ \midrule
    Swiss & TEar vs NP & -0.75 & (0.06) & 0.00 & -0.06 & (0.01) & 0.00 & 0.67 & (0.06) & 0.00 & -0.02 & (0.01) & 0.00\\
   Long term permit & TEar vs NP & -0.59 & (0.06) & 0.00 & 0.11 & (0.01) & 0.00 & 0.74 & (0.07) & 0.00 & 0.05 & (0.01) & 0.00\\
   \midrule
    Swiss & BC vs NP & -1.78 & (0.07) & 0.00 & -0.04 & (0.01) & 0.00 & -0.08 & (0.07) & 0.27 & -0.03 & (0.01) & 0.00\\
    Long term permit & BC vs NP & -1.68 & (0.07) & 0.00 & 0.07 & (0.01) & 0.00 & 0.01 & (0.08) & 0.86 & 0.06 & (0.01) & 0.00\\
    \midrule
   Swiss & TC vs NP & -1.72 & (0.11) & 0.00 & -0.03 & (0.01) & 0.00 & 0.23 & (0.12) & 0.04 & -0.01 & (0.01) & 0.45\\
    Long term permit & TC vs NP & -1.62 & (0.11) & 0.00 & 0.06 & (0.02) & 0.00 & 0.26 & (0.12) & 0.03 & 0.02 & (0.02) & 0.41\\
    \midrule
    Swiss & TE vs NP & -1.40 & (0.12) & 0.00 & -0.06 & (0.01) & 0.00 & 0.09 & (0.13) & 0.50 & -0.04 & (0.01) & 0.00\\
    Long term permit & TE vs NP & -1.21 & (0.12) & 0.00 & 0.13 & (0.02) & 0.00 & 0.20 & (0.13) & 0.12 & 0.08 & (0.02) & 0.00\\
\midrule
&&  \multicolumn{12}{c}{\textbf{Outcome: Earnings}} \\ \midrule
     Swiss & TEar vs NP & -407 & (37.70) & 0.00 & -407 & (37.70) & 0.00 & -307 & (64.43) & 0.00 & -307 & (64.43) & 0.00\\
    Long term permit & TEar vs NP & 818 & (75.74) & 0.00 & 818 & (75.74) & 0.00 & 617 & (129.42) & 0.00 & 617 & (129.42) & 0.00\\
        \midrule
     Swiss & BC vs NP & -338 & (40.17) & 0.00 & -338 & (40.17) & 0.00 & -287 & (66.98) & 0.00 & -287 & (66.98) & 0.00\\
    Long term permit & BC vs NP & 680 & (80.68) & 0.00 & 680 & (80.68) & 0.00 & 576 & (134.53) & 0.00 & 576 & (134.53) & 0.00\\
\midrule
     Swiss & TC vs NP & -332 & (62.99) & 0.00 & -332 & (62.99) & 0.00 & -238 & (88.69) & 0.01 & -238 & (88.69) & 0.01\\
    Long term permit & TC vs NP & 667 & (126.52) & 0.00 & 667 & (126.52) & 0.00 & 479 & (178.13) & 0.01 & 479 & (178.13) & 0.01\\
    \midrule
     Swiss & TE vs NP & -437 & (79.40) & 0.00 & -437 & (79.40) & 0.00 & -470 & (103.29) & 0.00 & -470 & (103.29) & 0.00\\
    Long term permit & TE vs NP & 879 & (159.46) & 0.00 & 879 & (159.46) & 0.00 & 944 & (207.45) & 0.00 & 944 & (207.45) & 0.00\\
    \bottomrule
    \end{tabular}
    \begin{tablenotes}
\textit{Note:} The table shows the GATEs for the different programmes in comparison to no programme (NP: Non Participation, TE: Temporary Earnings, BC: Basic courses, TC: Training Courses, TEMP: Temporary Employment) and the different sub-groups. Columns (3) to (5) show the results for the first year, namely the lock-in period, and columns (6) to (9) show it for the third year. 
\end{tablenotes}
\end{threeparttable}
\end{adjustbox}
\end{table}

==> Tables_results/GATES_tables/only_gates_language.tex <==

\begin{table}[htbp!]
\begin{adjustbox}{width=0.95\columnwidth, center}
\begin{threeparttable}
  \captionsetup{font=large}
    \caption{GATE for Proficiency in the local language, Swiss+ sample}
    \label{table:merged}
    \centering
    \begin{tabular}{@{}ll|rrrrrr|rrrrrrr@{}}
    \toprule
    \multicolumn{2}{l}{\textbf{Proficiency Local Language}} & \multicolumn{6}{c}{\textbf{First Year}} & \multicolumn{6}{c}{\textbf{Third Year}} \\
    \midrule
     & Programme & GATE & S.E. & p-value & GATE-ATE & S.E. & p-value & GATE & S.E. & p-value & GATE-ATE & S.E. & p-value \\
    \midrule
       &&  \multicolumn{12}{c}{\textbf{Outcome: Employment}} \\ \midrule
1 - basic knowledge & TEar vs NP & -0.60 & (0.06) & 0.00 & -0.60 & (0.06) & 0.00 & 0.78 & (0.07) & 0.00 & 0.78 & (0.07) & 0.00\\
    2 & TEar vs NP & -0.59 & (0.06) & 0.00 & -0.59 & (0.06) & 0.00 & 0.79 & (0.07) & 0.00 & 0.79 & (0.07) & 0.00\\
2  & TEar vs NP & -0.60 & (0.06) & 0.00 & -0.60 & (0.06) & 0.00 & 0.77 & (0.07) & 0.00 & 0.77 & (0.07) & 0.00\\
    4 & TEar vs NP & -0.61 & (0.06) & 0.00 & -0.61 & (0.06) & 0.00 & 0.76 & (0.07) & 0.00 & 0.76 & (0.07) & 0.00\\
    5 & TEar vs NP & -0.63 & (0.06) & 0.00 & -0.63 & (0.06) & 0.00 & 0.76 & (0.07) & 0.00 & 0.76 & (0.07) & 0.00\\
    6 & TEar vs NP & -0.66 & (0.06) & 0.00 & -0.66 & (0.06) & 0.00 & 0.72 & (0.07) & 0.00 & 0.72 & (0.07) & 0.00\\
    
    7 - mother tongue & TEar vs NP & -0.81 & (0.06) & 0.00 & -0.81 & (0.06) & 0.00 & 0.63 & (0.06) & 0.00 & 0.63 & (0.06) & 0.00\\ \midrule
    1 - basic knowledge & BC vs NP & -1.75 & (0.07) & 0.00 & -1.75 & (0.07) & 0.00 & 0.09 & (0.09) & 0.28 & 0.09 & (0.09) & 0.28\\
    2 & BC vs NP & -1.73 & (0.07) & 0.00 & -1.73 & (0.07) & 0.00 & 0.09 & (0.09) & 0.30 & 0.09 & (0.09) & 0.30\\
    3 & BC vs NP & -1.75 & (0.07) & 0.00 & -1.75 & (0.07) & 0.00 & 0.08 & (0.08) & 0.36 & 0.08 & (0.08) & 0.36\\
    4 & BC vs NP & -1.73 & (0.07) & 0.00 & -1.73 & (0.07) & 0.00 & 0.07 & (0.08) & 0.41 & 0.07 & (0.08) & 0.41\\
    5 & BC vs NP & -1.73 & (0.07) & 0.00 & -1.73 & (0.07) & 0.00 & 0.05 & (0.08) & 0.51 & 0.05 & (0.08) & 0.51\\
    6 & BC vs NP & -1.74 & (0.07) & 0.00 & -1.74 & (0.07) & 0.00 & 0.01 & (0.08) & 0.90 & 0.01 & (0.08) & 0.90\\
    7 - mother tongue & BC vs NP & -1.84 & (0.07) & 0.00 & -1.84 & (0.07) & 0.00 & -0.08 & (0.07) & 0.27 & -0.08 & (0.07) & 0.27\\
    \midrule
   1 - basic knowledge & TC vs NP & -1.62 & (0.12) & 0.00 & -1.62 & (0.12) & 0.00 & 0.05 & (0.13) & 0.69 & 0.05 & (0.13) & 0.69\\
    2 & TC vs NP & -1.60 & (0.11) & 0.00 & -1.60 & (0.11) & 0.00 & 0.09 & (0.13) & 0.50 & 0.09 & (0.13) & 0.50\\
    3 & TC vs NP & -1.60 & (0.11) & 0.00 & -1.60 & (0.11) & 0.00 & 0.08 & (0.13) & 0.54 & 0.08 & (0.13) & 0.54\\
    4 & TC vs NP & -1.58 & (0.11) & 0.00 & -1.58 & (0.11) & 0.00 & 0.09 & (0.13) & 0.48 & 0.09 & (0.13) & 0.48\\
    5 & TC vs NP & -1.59 & (0.11) & 0.00 & -1.59 & (0.11) & 0.00 & 0.12 & (0.12) & 0.34 & 0.12 & (0.12) & 0.34\\
    6 & TC vs NP & -1.57 & (0.11) & 0.00 & -1.57 & (0.11) & 0.00 & 0.12 & (0.12) & 0.30 & 0.12 & (0.12) & 0.30\\
    7 - mother tongue & TC vs NP & -1.63 & (0.11) & 0.00 & -1.63 & (0.11) & 0.00 & 0.10 & (0.11) & 0.37 & 0.10 & (0.11) & 0.37\\
    \midrule
    1 - basic knowledge & TE vs NP & -1.41 & (0.12) & 0.00 & -1.41 & (0.12) & 0.00 & 0.40 & (0.14) & 0.00 & 0.40 & (0.14) & 0.00\\
    2 & TE vs NP & -1.43 & (0.12) & 0.00 & -1.43 & (0.12) & 0.00 & 0.38 & (0.13) & 0.00 & 0.38 & (0.13) & 0.00\\
    3 & TE vs NP & -1.42 & (0.12) & 0.00 & -1.42 & (0.12) & 0.00 & 0.36 & (0.14) & 0.01 & 0.36 & (0.14) & 0.01\\
    4 & TE vs NP & -1.47 & (0.12) & 0.00 & -1.47 & (0.12) & 0.00 & 0.35 & (0.13) & 0.01 & 0.35 & (0.13) & 0.01\\
    5 & TE vs NP & -1.47 & (0.12) & 0.00 & -1.47 & (0.12) & 0.00 & 0.35 & (0.13) & 0.01 & 0.35 & (0.13) & 0.01\\
    6 & TE vs NP & -1.55 & (0.12) & 0.00 & -1.55 & (0.12) & 0.00 & 0.30 & (0.13) & 0.02 & 0.30 & (0.13) & 0.02\\
    7 - mother tongue & TE vs NP & -1.71 & (0.13) & 0.00 & -1.71 & (0.13) & 0.00 & 0.16 & (0.13) & 0.20 & 0.16 & (0.13) & 0.20\\
    \midrule
       &&  \multicolumn{12}{c}{\textbf{Outcome: Earnings}} \\ \midrule
    1 - basic knowledge & TEar vs NP & -4055 & (361) & 0.00 & 1888 & (192) & 0.00 & 3008 & (667) & 0.00 & 1173 & (253) & 0.00\\
    2 & TEar vs NP & -4171 & (397) & 0.00 & 1771 & (165) & 0.00 & 2964 & (825) & 0.00 & 1129 & (222) & 0.00\\
    3 & TEar vs NP & -4177 & (365) & 0.00 & 1766 & (184) & 0.00 & 3006 & (675) & 0.00 & 1172 & (232) & 0.00\\
    4 & TEar vs NP & -4447 & (407) & 0.00 & 1495 & (142) & 0.00 & 2874 & (866) & 0.00 & 1039 & (202) & 0.00\\
    5 & TEar vs NP & -4685 & (392) & 0.00 & 1257 & (120) & 0.00 & 2814 & (848) & 0.00 & 980 & (168) & 0.00\\
    6 & TEar vs NP & -5441 & (472) & 0.00 & 501 & (62) & 0.00 & 2209 & (848) & 0.01 & 374 & (128) & 0.00\\
    7 - mother tongue & TEar vs NP & -6469 & (454) & 0.00 & -527 & (47) & 0.00 & 1468 & (747) & 0.05 & -366 & (66) & 0.00\\
      \midrule
    1 - basic knowledge & BC vs NP & -8798 & (407) & 0.00 & 1623 & (198) & 0.00 & -479 & (723) & 0.51 & 1377 & (274) & 0.00\\
    2 & BC vs NP & -8876 & (434) & 0.00 & 1545 & (172) & 0.00 & -578 & (867) & 0.51 & 1279 & (241) & 0.00\\
    3 & BC vs NP & -8995 & (408) & 0.00 & 1426 & (183) & 0.00 & -569 & (729) & 0.44 & 1288 & (249) & 0.00\\
    4 & BC vs NP & -9141 & (438) & 0.00 & 1280 & (141) & 0.00 & -736 & (904) & 0.42 & 1121 & (211) & 0.00\\
    5 & BC vs NP & -9334 & (427) & 0.00 & 1087 & (118) & 0.00 & -832 & (888) & 0.35 & 1024 & (177) & 0.00\\
    6 & BC vs NP & -9998 & (490) & 0.00 & 423 & (62) & 0.00 & -1544 & (884) & 0.08 & 313 & (130) & 0.02\\
    7 - mother tongue & BC vs NP & -10865 & (475) & 0.00 & -444 & (48) & 0.00 & -2241 & (789) & 0.00 & -384 & (70) & 0.00\\
      \midrule
    1 - basic knowledge & TC vs NP & -7954 & (627) & 0.00 & 1438 & (327) & 0.00 & -149 & (944) & 0.87 & 509 & (427) & 0.23\\
    2 & TC vs NP & -8065 & (634) & 0.00 & 1327 & (279) & 0.00 & -142 & (1056) & 0.89 & 516 & (362) & 0.15\\
    3 & TC vs NP & -8092 & (623) & 0.00 & 1300 & (288) & 0.00 & -33 & (938) & 0.97 & 625 & (385) & 0.10\\
    4 & TC vs NP & -8287 & (633) & 0.00 & 1105 & (219) & 0.00 & -96 & (1074) & 0.93 & 562 & (298) & 0.06\\
    5 & TC vs NP & -8501 & (633) & 0.00 & 891 & (185) & 0.00 & 19 & (1060) & 0.99 & 677 & (257) & 0.01\\
    6 & TC vs NP & -9105 & (700) & 0.00 & 288 & (86) & 0.00 & -469 & (1083) & 0.66 & 189 & (150) & 0.21\\
    7 - mother tongue & TC vs NP & -9767 & (730) & 0.00 & -374 & (76) & 0.00 & -847 & (1037) & 0.41 & -189 & (101) & 0.06\\
      \midrule
    1 - basic knowledge & TE vs NP & -6864 & (657) & 0.00 & 2678 & (417) & 0.00 & 449 & (958) & 0.64 & 2217 & (497) & 0.00\\
    2 & TE vs NP & -7104 & (670) & 0.00 & 2437 & (364) & 0.00 & 243 & (1070) & 0.82 & 2011 & (426) & 0.00\\
    3 & TE vs NP & -7180 & (656) & 0.00 & 2361 & (382) & 0.00 & 186 & (963) & 0.85 & 1954 & (452) & 0.00\\
    4 & TE vs NP & -7688 & (688) & 0.00 & 1853 & (296) & 0.00 & -115 & (1107) & 0.92 & 1653 & (352) & 0.00\\
    5 & TE vs NP & -7896 & (708) & 0.00 & 1645 & (249) & 0.00 & -187 & (1107) & 0.87 & 1580 & (298) & 0.00\\
    6 & TE vs NP & -9011 & (830) & 0.00 & 530 & (101) & 0.00 & -1123 & (1173) & 0.34 & 645 & (157) & 0.00\\
    7 - mother tongue & TE vs NP & -10219 & (901) & 0.00 & -678 & (102) & 0.00 & -2378 & (1163) & 0.04 & -610 & (120) & 0.00\\
    \bottomrule
    \end{tabular}
\begin{tablenotes}
\textit{Note:} The table shows the GATEs for the different programmes in comparison to no programme (NP: Non Participation, TE: Temporary Earnings, BC: Basic courses, TC: Training Courses, TEMP: Temporary Employment) and the different sub-groups (1 - basic knowledge to 7 - mother tongue). Columns (3) to (5) show the results for the first year, namely the lock-in period, and columns (6) to (9) show it for the third year. 
\end{tablenotes}
\label{table:only_gate_language}
\end{threeparttable}
\end{adjustbox}
\end{table}

